Provably Efficient Reinforcement Learning for Adversarial Restless Multi-Armed Bandits with Unknown Transitions and Bandit Feedback

Restless multi-armed bandits (RMAB) play a central role in modeling sequential decision making problems under an instantaneous activation constraint that at most B arms can be activated at any decision epoch. Each restless arm is endowed with a state that evolves independently according to a Markov decision process regardless of being activated or not. In this paper, we consider the task of learning in episodic RMAB with unknown transition functions and adversarial rewards, which can change arbitrarily across episodes. Further, we consider a challenging but natural bandit feedback setting that only adversarial rewards of activated arms are revealed to the decision maker (DM). The goal of the DM is to maximize its total adversarial rewards during the learning process while the instantaneous activation constraint must be satisfied in each decision epoch. We develop a novel reinforcement learning algorithm with two key contributors: a novel biased adversarial reward estimator to deal with bandit feedback and unknown transitions, and a low-complexity index policy to satisfy the instantaneous activation constraint. We show $\tilde{\mathcal{O}}(H\sqrt{T})$ regret bound for our algorithm, where $T$ is the number of episodes and $H$ is the episode length. To our best knowledge, this is the first algorithm to ensure $\tilde{\mathcal{O}}(\sqrt{T})$ regret for adversarial RMAB in our considered challenging settings.

==> Analysis.tex <==
\section{Analysis}\label{sec:analysis}
Within this section, we present the theoretical outcomes achieved by \texttt{OARMAB-UCB}, focusing on cumulative regret defined in \eqref{eq:regret}. The primary technical challenges in bounding the cumulative regret come from two aspects. 
First, due to the index-based policy used in the considered adversarial RMAB setting, the conventional regret analysis in adversarial MDPs\citep{rosenberg2019online, jin2020learning} and CMDPs \citep{qiu2020upper} focusing on the occupancy measure cannot be directly used. Second, compared with the stochastic RMAB setting \cite{xiong2022AAAI, xiong2022Neurips} with fixed reward distributions, a major difference is that the best-in-hindsight policy for all episodes in the adversarial setting does not guarantee the highest reward for every individual episode as in the stochastic setting. Thus, both positive and negative regret might occur in each episode, which renders the regret decomposition among episodes in a stochastic setting not applicable to our adversarial setting. 


In the following, we first illustrate the final theoretical result in Theorem \ref{thm:regret} and then provide details on proving it. 

\begin{theorem}\label{thm:regret}
With probability at least $1-3\epsilon$,
the regret of \texttt{OARMAB-UCB} policy with $\eta=\sqrt{\frac{\ln(|\cS|^2|\cA|)}{T}}$ satisfies 
\begin{align}\label{eq:regret_thm}
&\Delta(T)=\tilde{\mathcal{O}}\Bigg(NH\sqrt{T\ln(|\cS|^2|\cA|)}\nonumber\\
&+\!\!\sqrt{2}H\sqrt{\!NT\ln\frac{4|\cS||\cA|NT}{\epsilon}}\!+\!B\sqrt{|\cS||\cA|NTH}\Bigg).
\end{align}
\end{theorem}


\begin{remark}
The regret in \eqref{eq:regret_thm} contains three major parts, which represent three different sources for regret. The first term is regret due to the OMD online optimization for occupancy measure updates, the second term represents the regret due to bandit-feedback of adversarial rewards, and the third term comes from the employment of the proposed RMI index policy to the RMAB setting. The overall regret is dominated by the order of $\mathcal{O}(H\sqrt{T})$, which is same as the conventionl adversarial MDP and CMDP settings \citep{rosenberg2019online, jin2020learning,qiu2020upper}. However, the regret order is $\sqrt{H}$ times worse than the stochastic RMAB settings as \citep{xiong2022AAAI, xiong2022Neurips}.
The main reason is due to the varying adversarial rewards which are bandit -feedback, and thus it requires an estimation and online optimization procedure.
    {The key contribution and novelty of our proposed RL algorithm is to leverage our proposed RMI index policy for making decisions, rather than directly contending with an extremely large state-action space to balance between exploration and exploitation.  These together contribute to the sub-linear regret of with a low complexity.}
\end{remark}

\subsection{Proof of Theorem \ref{thm:regret}}

As aforementioned, the challenge for showing Theorem \ref{thm:regret} lies in two aspects, i.e., 1) \textbf{how to connect the index-based policy in the RMAB setting with the occupancy measure defined in \eqref{eq:OM}}, and 2) \textbf{how to get rid of the non-decomposable regret due to adversarial reward.} In the following, we first present the upper bound of the original problem in \eqref{eq:orginal_P} in the following lemma.
\begin{lemma}\label{lem:upperbound}
There exists a set of occupancy measures $\mu_{\pi}^*:=\{\mu^*_n(s,a;h), \forall n\in[N], s\in\cS, a\in\cA, h\in[h]\}$ under policy $\pi$  that optimally solve \eqref{eq:orginal_P} with a relaxed constraint in \eqref{eq:relaxed_constraint}. In addition, $\sum_{t=1}^T \langle{\mu_\pi^*}, r^t\rangle$ is no less than $R( T, \pi^{opt})$, where $\mu_\pi^*$ is the stacked vector of all occupancy measures $\mu_n^*(s,a;h)$ and $r^t$ is the stacked vector of all rewards $r_n^t(s,a)$ for all $n, s, a$.
\end{lemma}

Lemma \ref{lem:upperbound} indicates that the occupancy measure-based solution to the \eqref{eq:orginal_P} with a relaxed constraint can always provide an upper bound of the optimal reward $R( T, \pi^{opt})$ achieved by best-in-hindsight policy $\pi^{opt}$ of the original problem \eqref{eq:orginal_P}. Provided Lemma \ref{lem:upperbound}, we have the following lemma to decompose the total regret $\Delta(T)$.




\begin{lemma}\label{lemma:regret_decomp}
Denote $\pi^{\mu^*}$ as the optimal policy for the original problem with relaxed constraint $\mathbb{E}_{\pi}\left[\sum_{n=1}^N A_n^{t,h}\right]\leq B,h\in[H], t\in[T]$, and $\{\tilde{\pi}^t, \forall t\}$ are polices executed on the virtual MDPs at each episode selected from the plausible MDP set.
The regret in \eqref{eq:regret} can be upper bounded as
\begin{align}\label{eq:lemma2}
    \Delta(T)\leq &R( T, \pi^{\mu^*}, \{\hat{r}_n^t, \forall n\in[N], t\in[T]\})\nonumber\\
    &\underset{Term_1}{\underbrace{\qquad-R( T, \{\tilde{\pi}^t, \forall t\}, \{\hat{r}_n^t, \forall n\in[N], t\in[T]\})}}\nonumber\allowdisplaybreaks\\
    &+R( T, \{\tilde{\pi}^t, \forall t\}, \{\hat{r}_n^t, \forall n\in[N], t\in[T]\})\nonumber\\
    &\underset{Term_2}{\underbrace{\qquad-R( T, \{\tilde{\pi}^t, \forall t\}, \{{r}_n^t, \forall n\in[N], t\in[T]\})}}\nonumber\allowdisplaybreaks\\
    &+R( T, \{\tilde{\pi}^t, \forall t\}, \{{r}_n^t, \forall n\in[N], t\in[T]\})\nonumber\\&\underset{Term_3}{\underbrace{\qquad-R( T,\{\pi^t, \forall t\}, \{{r}_n^t, \forall n\in[N], t\in[T]\})}}. \allowdisplaybreaks
\end{align}
\end{lemma}



\begin{remark}
{\color{red}Notation mismatch. }
 The inequality in Lemma \ref{lemma:regret_decomp} is grounded on the fact that $R( T, \pi^{opt})$ is upper bounded by the optimal value of the relaxed fluid model, which is denoted as $\sum_{t=1}^T \langle \mu_{\pi}^*, r^t\rangle$, and the design of an overestimated reward estimator in \eqref{eq:reward_estimator}. The three terms in \eqref{eq:lemma2} account for the three sources of regret in Theorem \ref{thm:regret}. The goal for bounding regret $\Delta(T)$ is transferred  to bound each individual term respectively with the aid of Lemma \ref{lemma:regret_decomp}. 
\end{remark}



 

Specifically, $Term_1$ is the amount of regret majorly controlled by the OMD for online convex optimization, $Term_2$ is regret dominated by the bias of the reward estimator, and $Term_3$ is the regret due to the unknown transitions and optimistically search in a confidence ball.  Since OMD is used for updating the occupancy measure, to bound $Term_1$, the key is to connect items in $Term_1$ with the occupancy measure, which leverages the result in Lemma \ref{lem:upperbound}. In addition, due to the overestimation of the reward $\hat{r}_n^t$, $Term_2$ can be bounded. $Term_3$ is the regret directly related to the learned \texttt{OARMAB-UCB}, and thus we bound it based on the count of visits of each state-action pair, rather than the occupancy measure. The three terms are bounded separately in the following lemmas. 

\textbf{Regret due to OMD online optimization.}
\begin{lemma}\label{lem:term1}
With probability $1-2\epsilon$, $Term_1$ is upper bounded by
\begin{align*}
    Term_1\leq \frac{NH\ln(|\cS|^2|\cA|)}{\eta}+\eta{NH(T+1)}.
\end{align*}
\end{lemma}


\textbf{Regret due to Bandit-feedback Reward.}
\begin{lemma}\label{lem:term2}
With probability $1-3\epsilon$, $Term_2$ is upper bounded by
\begin{align*}
    Term_2\leq\sqrt{2}H\sqrt{\ln\frac{4|\cS||\cA|NT}{\epsilon}}\cdot \sqrt{NT}+HN\sqrt{TN\ln 1/\epsilon}.
\end{align*}
\end{lemma}

\textbf{Regret due to index policy.}
\begin{lemma}\label{lem:term3}
With probability $1-2\epsilon$, $Term_3$ is upper bounded by
\begin{align*}
    Term_3\leq\Big(\sqrt{2\ln\Big(\frac{4|\cS||\cA|NTH}{\epsilon}\Big)}+2B\Big)\sqrt{|\cS||\cA|NTH}
\end{align*}
\end{lemma}

Combining Lemma \ref{lem:term1}, Lemma \ref{lem:term2}, and Lemma \ref{lem:term3} yields the final result in Theorem \ref{thm:regret}. 














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{conclusion}
In this study, we introduce the initial efficient algorithm capable of achieving $\mathcal{O}(T)$ regret in the context of learning regret minimization in Adversarial RMABs when faced with unknown transition functions, adversarial losses, and bandit feedback. Our primary algorithmic innovation lies in the introduction of an index-based policy designed to confront optimism while utilizing the upper confidence ball.  An inherent open question in this pursuit pertains to the characterization of the lower bound in this challenging setting considered in our work.

==> Intro.tex <==
\section{Introduction}
Restless multi-armed bandits (RMABs) have proven to be invaluable for modeling a wide spectrum of sequential decision-making challenges. These applications encompass domains such as job scheduling, healthcare management, and queueing systems. Within the realm of RMABs, a collection of $N$ arms exists, and the individual state of each arm evolves independently in accordance with a two-action Markov Decision Process (MDP). When an arm is pulled at any given moment, its progression follows a stochastic path determined by one transition kernel, whereas, in the absence of pull, a different kernel governs its evolution.


Prior research predominantly focuses on the stochastic setting, in which rewards are generated during each transition following a deterministic distribution. The primary goal in this context is to maximize the expected cumulative reward, either over a finite horizon, infinite horizon, or episodic setting,   while abiding by constraints on the number of arms that can be activated at any given time moment. However, in real-world applications, the rewards might be determined by an adversary, changing over time, which makes the conventional techniques fail in such scenarios. 


Inspired by recent investigations into online resource allocations involving episodic MDPs commonly found in fields such as revenue management and online advertising, this paper considers the online learning approaches for RMABs under an adversarial reward setting, marking a pioneering exploration in this domain. In particular, we consider an episodic setting where the $N$ MDPs associated with each arm are initialized at the beginning of each episode.  The primary goal is to minimize the cumulative regret, which measures the amount of reward they lose in comparison to what they would have achieved by consistently following the best-in-hindsight policy that complies with constraints across all episodes.


We present an innovative algorithm tailored for the adversarial RMAB model, wherein the decision maker faces with an unknown transition function and rewards that exhibit arbitrary fluctuations over time, with bandit feedback as the reward source {\color{red}(where only the reward for each visited
state-action pair is revealed)}. In contrast to prior research involving adversarial MDPs and CMDPs, our algorithm, \texttt{ORMAB-UCB}, adopts an index-based policy, aligning it with the stochastic RMAB literature. Diverging from the traditional stochastic RMAB setting, we incorporate Online Mirror Descent (OMD) to address the challenges posed by online convex optimization in the face of adversarial rewards. To cope with the unknown dynamics, as represented by the stochastic transition function, we integrate techniques inspired by UCRL-2. We summarize our contributions as follows.

%$\bullet$ We present \texttt{ORMAB-UCB}, an index-aware online reinforcement learning (RL) algorithm designed specifically for episodic Restless Multi-Armed Bandits (RMAB) operating under an adversarial reward setting. \texttt{ORMAB-UCB} adopts an online learning approach, continuously updating its model as new samples become available. The algorithmic framework consists of two key stages: model construction and the subsequent implementation of an index policy-based solution. This algorithm is tailored to address an online convex optimization problem, incorporating the concept of an occupancy measure. This novel approach allows us to derive provably optimal index policies that play a crucial role in guiding decision-making during the exploitation phase.

%$\bullet$ The primary difficulty arises when dealing with bandit feedback, as the application of OMD necessitates the creation of reliable reward estimators due to the incomplete disclosure of the reward function. Due to the "hard" activation constraint of the considered RMABs, the conventional method of developing unbiased loss estimators through inverse occupancy measure becomes impractical in our context, the index-based policy will converge to the desired occupancy measure in a non-asymptotic region. We thus propose a new reward-estimator that is simply based on the number of visits of each state-action pari without any further greedy searching algorithm as in. The main idea is also to make an overestimated reward to encourage explorations.  

%$\bullet$ We present the first regret analysis for the episodic RMABs with adversarial rewards problem. Our analysis demonstrates that the unique design characteristics of \texttt{ORMAB-UCB} contribute to their regret scaling at approximately $\mathcal{O}(\sqrt{T})$, a polynomial dependency only on the number of arms and states.  

% \subsection{Motivating example 1: Revenue Management}

% \emph{Hotels and Airlines:} These industries receive requests for rooms or flights. They decide how to process these requests in real-time based on the availability of remaining rooms and flight seats. For instance, a hotel might receive a booking request for a specific type of room. Based on the current availability and predicted future demand, the hotel decides whether to accept the booking, offer an alternative, or decline the request. This decision-making process aims to maximize revenue by optimizing room allocations.



\textbf{Notations.}





==> Proposed_method.tex <==
\section{Reinforcement Learning Solution}\label{sec:learning}

In this section, we show the feasibility of designing a reinforcement learning (RL) algorithm to address the computationally challenging regret minimization problem as defined in \eqref{eq:regret}. To achieve this, we draw upon the widely recognized UCRL approach \citep{jaksch2010near} and introduce an episodic RL algorithm named \texttt{OARMAB-UCB}. Notably, \texttt{OARMAB-UCB} rigorously adheres to the "hard" activation constraint outlined in \eqref{eq:orginal_P} at every decision epoch. This adherence is made possible by utilizing a low-complexity index policy for decision-making during each decision epoch, making \texttt{OARMAB-UCB} computationally efficient. Before presenting the proposed \texttt{OARMAB-UCB} algorithm, we introduce a time-dependent occupancy measure, specifically designed for the considered episodic RMAB setting with multiple MDPs and "hard" activation constraint. 

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{Adversarial_RMAB_flow.pdf}
    \caption{The workflow of proposed \texttt{OARMAB-UCB} and its regret analysis. The dashed arrows present the aimed procedures for solving the original problem in \eqref{eq:orginal_P}, and the solid arrows shows the true procedures of the proposed \texttt{OARMAB-UCB}. By relaxing the "hard" activation constraint as shown in \eqref{eq:relaxed_constraint},  \texttt{OARMAB-UCB} updates occupancy measure via OMD as in \eqref{eq:UCB_extended}. Combined with the reward estimation in \eqref{eq:reward_estimator}, it establishes the RMI index policy in \eqref{eq:importance-index}. }

    \label{fig:Flowchart}
%     \vspace{-0.1in}
\end{figure*}


 
\subsection{A Time-Dependent Occupancy Measure}

Solving the problem with techniques from online learning requires introducing the concept of \emph{occupancy measures}~\citep{altman1999constrained}. Unlike the \emph{time-independent} occupancy measure defined in previous work \citep{rosenberg2019online,jin2020learning, qiu2020upper}, we define the \emph{time-dependent} occupancy measure to deal with the finite-horizon episodic setting. The occupancy measure $\mu$ of a policy $\pi$ in a finite-horizon MDP is defined as the expected number of visits to a state-action pair $(s, a)$ at each time step $h$ in each episode $t$.  Formally,
\begin{align}\label{eq:OM}
\mu^\pi=& \Big\{\mu_n(s,a;h)=\mathbb{P}(S_n^h=s, A_n^h=a)\nonumber\\
&\qquad: \forall n\in[N], s\in\cS, a\in\cA, h\in[H] \Big\}.
\end{align}
It can be easily checked that occupancy measures satisfy the following two properties. First, 
\begin{align}
\sum_{s\in\cS}\sum_{a\in\cA}\mu_n(s,a;h)=1, \forall n\in[N], h\in[H],
\end{align}
with $0\leq \mu_n(s,a;h)\leq 1$.  Hence the occupancy measure $\mu_n$, $\forall n$ is a probability measure. Second, the fluid balance exists in occupancy measures transitions as
\begin{align}
\sum_{a\in\mathcal{A}}\!\!\mu_n(s,a;h)\!=\!\!\sum_{s^\prime}\!\sum_{ a^\prime}\!\mu_n(s^\prime, a^\prime; h-1)P_n(s^\prime, a^\prime,s)
\end{align}
It turns out that these two properties suffice for any function $\mu^\pi: X\times A \rightarrow [0,1]$ to be an occupancy measure associated with some transition function and some policy $\pi$.

A key distinction lies in our proposed occupancy measure in \eqref{eq:OM}, which is specifically designed to account for the finite-time horizon RMAB setting, rendering it time-dependent. In contrast, the conventional approaches for MDPs \citep{rosenberg2019online, jin2020learning} and CMDPs \citep{qiu2020upper} rely on a time-independent occupancy measure. Furthermore, the conventional method typically leverages the stationary policy derived from the occupancy measure, while our unique challenge stems from the imposition of a stringent "hard" activation constraint, making the utilization of a stationary policy unfeasible in our context. 

\begin{remark}
In particular, by defining time-independent occupancy measure $q(s,a), \forall s, a$ for a single MDP in \citep{rosenberg2019online, jin2020learning, qiu2020upper}, the regret of can be directly expressed as $\sum_{t=1}^T\langle q_t-q^*, \ell_t\rangle$ with $q_t$ being the vectors of stacked occupancy measure under policy $\pi^t$ in the $t$-th episode, $q^*$ being the stacked occupancy measure under the best-in-hindsight policy for all $T$ episodes, and $\ell_t$ being the vector of stacked adversarial loss values in the $t$-th episode (Note that the notations in this remark exactly come from previous work). This is guaranteed by the stationary policy derived from the occupancy measures $q_t$ at each episode $t$. Hence, characterizing the regret is only determined by those learned occupancy measures. However, in the considered RMAB setting, since there is no such stationary policy due to the "hard" activation constraint and thus relying on some index-based policies, the regret characterization of \eqref{eq:regret} considered in this paper cannot be directly linked with the defined occupancy measures in \eqref{eq:OM}, which adds additional challenge to characterize the regret bound. 
\end{remark}



\subsection{Overview of \texttt{OARMAB-UCB} }\label{sec:learning-alg}


% \begin{figure}
%     \centering
%     \includegraphics[width=1\textwidth]{Workflow.pdf}
%     \caption{The workflow of proposed \texttt{OARMAB-UCB} and comparison of conventional adversarial CMDPs and MDPs.}
%     \label{fig:Flowchart}
% %     \vspace{-0.1in}
% \end{figure}


The complete pseudocode of our algorithm, \texttt{OARMAB-UCB},
is presented in Algorithm \ref{alg:UCB}, which consists four key components: 1) maintaining a confidence set of the
transition function by adapting the upper confidence bound (UCB) strategy \citep{auer2002finite}, 
2) constructing adversarial reward estimators, 3) relaxing the "hard" activation constraint in \eqref{eq:orginal_P} with the use of occupancy measure, 4) using Online Mirror Descent (OMD) to update
the occupancy measure,   and 5) designing index-based policy according to the updated occupancy measure. 
   Specifically, \texttt{OARMAB-UCB} runs in an episodic manner with total $T$ episodes and each episode containing $H$ consecutive slots.  We denote the $t$-th episode by $\mathcal{H}_t$ and let $\tau_t:= H(t-1)+1$ denote the time when it starts. 



\subsubsection{Upper Confidence Set}




\texttt{OARMAB-UCB} constructs a confidence ball that contains a set of plausible MDPs \citep{jaksch2010near, xiong2022AAAI,xiong2022Neurips}  for each arm $n\in\mathcal{N}$ to encourage exploration.
In particular, \texttt{OARMAB-UCB} maintains two counts for each user $n$.  Let $C_n^{t-1}(s,a), \forall n\in[N]$ be the number of visits to state-action pairs $(s,a)$ until $\tau_t$, and $C_n^{t-1}(s,a, s^\prime), \forall n\in[N]$ be the number of transitions from $s$ to $s^\prime$ under action $a$. At $\mathcal{H}_t$, \texttt{OARMAB-UCB} updates the respective counts $\forall (s,a,s^\prime)\in\mathcal{S}\times\mathcal{A}\times\mathcal{S}$ as
\begin{align*}
    C_n^{t}(s,a)&=C_n^{t-1}(s,a)+\sum_{h=1}^{H}\mathds{1}(S_n^{t,h}=s,A_n^{t,h}=a),\\
    C_n^{t}(s,a, s^\prime)&=C_n^{t-1}(s,a, s^\prime)\\
    &+\sum_{h=1}^{H}\mathds{1}(S_n^{t,h+1}=s^\prime|S_n^{t,h}=s,A_n^{t,h}=a),
\end{align*}
where $S_n^{t,h}$ is the state of arm $n$ at the $h$-th time slot in episode $t$. 
At $\tau_t,$ \texttt{OARMAB-UCB}  estimates the true transition model  by the corresponding empirical averages as:
\begin{align}\label{eq:empirical_est_P}
\hat{P}_n^{t}(s^\prime|s,a)=\frac{C_n^{t-1}(s,a,s^\prime)}{\max\{C_n^{t-1}(s,a),1\}}.
\end{align}
The \texttt{OARMAB-UCB} further defines confidence intervals for the transition probabilities  such that the true transition probabilities  lie in them with high probabilities.  Formally, for $\forall (s,a)\in\mathcal{S}\times\mathcal{A}$, we define
\begin{align}\label{eq:confidence_ball} 
 \cP_n^{t}(s,a)&:=\{\tilde{P}_n^t(s^\prime|s,a),\forall s^\prime:\nonumber\\
 &\quad\quad|\tilde{P}_n^t(s^\prime|s,\!a)\!-\!\hat{P}_n^{t}(s^\prime|s,\!a)|\!\leq\! \delta_n^{t}(s,\!a)\},
\end{align}
where the size of the confidence intervals $\delta_n^{t}(s,a)$ is built according to the Hoeffding inequality \citep{maurer2009empirical} for $\epsilon\in(0,1)$ as
\begin{align}
\delta_n^{t}(s,a)\!=\!\sqrt{\frac{1}{2C_n^{t-1}(s,a)}\!\log\!\Big(\frac{4|\cS||\cA|N(t\!-\!1)H}{\epsilon}\Big)}.
\end{align}




\begin{algorithm}[t]
	\caption{\texttt{OARMAB-UCB} Policy}
	\label{alg:UCB}
	\begin{algorithmic}[1]
     \REQUIRE  Initialize $C_n^{1}(s,a)=0,$ and  $\hat{P}_n^{1}(s^\prime|s,a)=1/|\cS|$	
		\FOR{$t=1,2,\cdots,T$}
		%\If{$h=1$}
	 \STATE Construct $\cP_n^{t}(s,a)$   according to \eqref{eq:confidence_ball} at $\tau_t$; 		
		%\EndIf
  \STATE Estimate the adversarial reward $\hat{r}_n^t(s,a), \forall s\in\cS, a\in\cA, n\in[N]$ according to \eqref{eq:reward_estimator};
    \STATE Relax the "hard" activation constraint in \eqref{eq:orginal_P} to  \eqref{eq:relaxed_constraint} by using occupancy measure;
		\STATE Compute the optimal solution \eqref{eq:UCB_extended};
	   \STATE Recover $\xi^{t,\star}$ according to \eqref{eq:final-policy-learned} and establish the corresponding indices $\pi^{t,\star}$;
		\STATE Execute $\pi^{t,\star}$ in the current episode.
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

\subsubsection{Adversarial Reward Estimators}
\label{sec:estimator}
{ 
A frequently employed strategy for addressing partial information feedback in adversarial online learning scenarios, like those found in adversarial MAB problems\citep{rosenberg2019b, jin2020learning}, involves creating loss estimations using observed data. Specifically, inverse importance-weighted estimators are extensively utilized for this purpose.
For our problem, with a trajectory for episode $t$,
we leverage similar idea and propose an estimator $\hat{r}_n^{t}(s,a)$ for adversarial reward as
\begin{align}\label{eq:reward_estimator}\nonumber
    \hat{r}_n^{t}(s,a)&=
\min\left(\Bigg(\frac{r_n(s,a)}{\max\{c_n^{t}(s,a),1\}/H}+\delta_n^t(s,a)\right)\nonumber\allowdisplaybreaks\\
&\qquad\qquad\qquad\quad\mathds{1}(\exists h, S_n^{t,h}=\!s, A_n^{t,h}=\!a),1\Bigg)\nonumber\allowdisplaybreaks\\
&\qquad+(1-\mathds{1}(\exists h, S_n^{t,h}=\!s, A_n^{t,h}=\!a),
\end{align}
where $c_n^t$ is the number of visits to state-action pair $(s,a)$ in episode $t$.
Clearly, $\frac{r_n(s,a)\mathds{1}(\exists h, S_n^{t,h}=s, A_n^{t,h}=a)}{\max\{c_n^{t}(s,a),1\}/H}$ is an unbiased estimator of ${r}_n^{t}(s,a)$. We add a bonus term $\delta_n^t(s,a)$ to encourage explorations. The reward estimator in \eqref{eq:reward_estimator} guarantees that $\hat{r}_n^t(s,a)$ is always an overestimation of $r_n^t(s,a), \forall s, a, n, t$ and is upper bounded by $1$, which is beneficial for the regret characterization in the subsequent section. }

\textbf{Difference with stochastic RMAB setting .} 
As the rewards are generated according to a fixed stochastic distribution in stochastic setting\citep{xiong2022AAAI, xiong2022Neurips}, the reward estimator is usually the sample mean, i.e.,
$\hat{r}_n^{t}(s,a)=
\frac{\sum\limits_{\tau=1}^{t-1}\sum\limits_{h=1}^{H}r_n(s,a)\mathds{1}(S_n^{\tau,h}=s, A_n^{\tau,h}=a)}{\max\{C_n^{t-1}(s,a),1\}}, \forall s,a,n.$ This is fundamentally different from the adversarial setting considered in this paper where the rewards are determined by an adversary, changing over episodes. Thus, the rewards of those unobserved state-action pairs will not revealed at the current episode due to bandit-feedback and will change in the next episode, which imposes a great challenge on designing policies and characterizing the associated regret.


\textbf{Difference with adversarial MDP setting.} In the adversarial setting \citep{rosenberg2019b, jin2020learning}, a common importance-weighted estimator of the loss is $\hat{\ell}^t(s,a)=\frac{\ell^t(s,a)\mathds{1}(\exists h, S_n^{t,h}=s, A_n^{t,h}=a)}{q^{\pi_t}(x,a)}$ with $q^{\pi_t}(s,a)$ being the converged stationary occupancy measure under policy $\pi_t$, which is unbiased. Due to the unknown transitions, \citep{jin2020learning} proposed an underestimated estimator by greedily searching occupancy measure from the confidence ball to replace $q^{\pi_t}(s, a)$. However, this search requires an additional effort and cannot be directly applied to our RMAB setting as we cannot directly use policies in \citep{jin2020learning} to guarantee the "hard" activation constraints
in RMAB problems, and hence we cannot guarantee that the estimator is an overestimation or an underestimation of the true rewards. Given these difficulties, we propose the novel estimator in \eqref{eq:reward_estimator} which is easy to compute and an overestimator of the original reward functions. 

\subsubsection{Relaxed"hard" activation constraint}
The most challenging part for dealing with RMAB problem even in stochastic setting comes from the "hard" activation constraint in \eqref{eq:orginal_P}. A common way is to  relax the "hard" activation constraint to a constraint that is satisfied in average first as proposed by \citep{whittle1988restless}, i.e.,
\begin{align}\label{eq:relaxed_constraint}
    \mathbb{E}_{\pi}\left[\sum_{n=1}^N A_n^{t,h}\right]\leq B ,h\in[H], t\in[T],
\end{align}
and then design an index-based policy (i.e., Whittle index policy) by solving the original  problem \eqref{eq:orginal_P} with relaxed constraint in \eqref{eq:relaxed_constraint} to satisfy the orginal "hard" activation constraint at each decision epoch. 
With the aid of occupancy measure defined in \eqref{eq:OM}, the relaxed constraint in \eqref{eq:relaxed_constraint} for the online learning problem in \eqref{eq:regret} can be further expressed as
\begin{align}\label{eq:relax_constraint2}
    \sum_{n=1}^N\sum_{s,a}a\mu_n^t(s,a;h)\leq B, \forall h\in[H], t\in[T].
\end{align}


\subsubsection{Occupancy Measure Update}
Given the plausible confidence set and the estimated rewards,  \texttt{OARMAB-UCB} computes a policy $\pi^{t,\star}$ by  solving an optimistic planning problem where the MDP parameters can be chosen
from the constructed confidence ball.
To this end, we leverage the \textit{state-action-state occupancy measure} $z_n^t(s, a, s^\prime; h)$ defined as $z_n^t(s, a, s^\prime; h)=P_n(s^\prime|s,a)\mu_n^t(s,a;h)$ to express the confidence intervals of the transition probabilities.  Similar to \citep{rosenberg2019online, jin2020learning}, we leverage the idea of OMD for online convex optimization to force that the updated occupancy measure in the current episode does not stray too far from the previously selected occupancy measure in the last episode.
Hence, we have the following optimization problem over $z^t:=\{z_n^t(s, a, s^\prime; h), \forall n\in[N]\}$: 
\begin{align}\label{eq:UCB_extended}
\max_{z^t}&\sum_{h=1}^{H}\sum_{n=1}^{N}\sum_{(s,a,s^\prime)}\!\!\! \eta z_n^t(s,a, s^\prime;h)\hat{r}_n^{t-1}(s,a)\!\!-\!\!D(z^t||z^{t-1})\nonumber\displaybreak[0]\\
\mbox{ s.t.} &\sum_{n=1}^{N}\sum_{(s,a,s^\prime)} az_n^t(s,a,s^\prime; h) \le B ,\quad~\forall h\in[H], \nonumber\displaybreak[1]\\
&{\sum_{a, s^\prime}} z_n^t(s,a,s^\prime;h)\!=\!\!\!\sum_{s^\prime, a^\prime}\!z_n^t(s^\prime, a^\prime, s; h-1),\forall h\!\in\![H],  \nonumber\displaybreak[2]\\ 
&~\frac{z_n^t(s,a,s^\prime;h)}{\sum_y z_n^t(s,a,y;h)}-(\hat{P}_n^t(s^\prime|s,a)+\delta_n^t(s,a))\leq 0, \nonumber\displaybreak[3]\\ 
&-\frac{z_n^t(s,a,s^\prime;h)}{\sum_y z_n^t(s,a,y;h)}\!+\!(\hat{P}_n^t(s^\prime|s,a)\!-\!\delta_n^t(s,a))\!\leq\! 0, \nonumber\\ 
& z_n^t(s,a, s^\prime;h)\!\geq\! 0,  \forall s,s^\prime\!\in\mathcal{S}, a\!\in\!\mathcal{A},\forall n\!\in\![N].
\end{align}
Notice that $\eta$ is a positive weight parameter and  $D(z^t||z^{t-1})$ is the unnormalized Kullback-Leible (KL) divergence between two occupancy measure defined as
\begin{align}\label{eq:KL_divergence}
\hspace{-0.3cm}D(z^t||z^{t-1})&:=\sum_{h=1}^{H}\sum_{s,a,s^\prime}z^t(s,a,s^\prime;h)\ln\frac{z^t(s,a,s^\prime;h)}{z^{t-1}(s,a,s^\prime;h)}\nonumber\\
&\qquad-z^t(s,a,s^\prime;h)+z^{t-1}(s,a,s^\prime;h).
\end{align}


\begin{remark}
    The significant departure from the stochastic RMAB setting \citep{xiong2022AAAI,xiong2022Neurips} stems from two key elements introduced in the adversarial setting: the incorporation of additional KL-divergence and the adoption of OMD for online optimization of the occupancy measure. These additions shift the nature of occupancy measure updates from the linear programming (LP) framework observed in the stochastic setting to a non-LP problem. Additionally, in the adversarial context\cite{rosenberg2019online, jin2020learning}, a noteworthy distinction arises in the form of an extra constraint, which serves to a relaxation of the originally stringent "hard" activation constraint. In the subsequent section, we will delve into the development of an index-based policy, grounded in the updated occupancy measure, with the objective of ensuring satisfaction with the "hard" activation constraint.
\end{remark}

\begin{remark}
This problem has $O(|\mathcal{S}|^2|\mathcal{A}|HN)$ constraints and decision variables and can be solved efficiently.
 Similar to \citep{rosenberg2019online}, we can first solve the unconstrained problem by setting $\tilde{z}^{t}(s,a,s^\prime; h)=z^{t-1}(s,a,s^\prime;h)e^{\eta \hat{r}^{t-1}(s,a)}$, and then project $\tilde{z}^{t}$ to the feasible set $\cZ^t$ defined by the constraints in \eqref{eq:UCB_extended}, which can be reduced to a convex optimization problem. We relegate the details in the supplementary materials.    Such an approach was also used in 
the context of adversarial MDPs \citep{jin2019learning,rosenberg2019online} and in constrained MDPs~\citep{kalagarla2020sample,efroni2020exploration}.
\end{remark}




\subsubsection{Index Policy Design}
 Once we compute the optimal solution $z^{t,\star}$ to~(\ref{eq:UCB_extended}), we recover the Markovian randomized policy $\xi_t^{\star}$ as
\begin{align}\label{eq:final-policy-learned}
\xi_n^{t,\star}(s,a;h)=\frac{\sum_{s^\prime}z_n^{t,\star}(s,a,s^\prime;h)}{\sum_{b,s^\prime}z_n^{t,\star}(s,b,s^\prime;h)},\quad \forall n\in[N].
\end{align}
However, the randomized policy in \eqref{eq:final-policy-learned} cannot be directly applied as conventional work in adversarial MDPs \citep{rosenberg2019online} and CMDPs \citep{qiu2020upper} due to the existence of the "hard" activation constraint in \eqref{eq:orginal_P}. To deal with the "hard" constraint,  we leverage the index policy-based idea in stochastic RMAB settings \citep{xiong2022AAAI, xiong2022Neurips} and introduce a novel index from the randomized policy in \eqref{eq:final-policy-learned}. Hence, the index policy ranks the indices of each arm at every time step and activates the $B$ arms with the largest indices to guarantee the "hard" active budget constraint. We name this type of policy as the reward-maximizing index (RMI) policy.  

\textbf{The RMI Policy.}
  Our proposed policy $\pi^{t,\star}:=\{\pi_{n}^{t,\star}, \forall n\}$ attaches the following index $\mathcal{I}_n^t(s;h)$ to each user $n$ in time slot $h$ for episode $t$, 
\begin{align}\label{eq:importance-index}
\mathcal{I}_n^t(s;h):=\xi^{t,\star}_n(s,1;h),\quad\forall n\in[N],
\end{align}
where $\xi^{t,\star}_n(s,a;h)$ is defined in~(\ref{eq:final-policy-learned}). Notice that the probability $\xi^{t,\star}_n(s,a;h)$ is related with the \textit{reward} of action $a$ in state $s$ in time slot $h$ towards the reward maximization, and is determined by the occupation measure derived by solving ~\eqref{eq:UCB_extended}.  Let $\mathcal{I}^t(h):=\{\mathcal{I}^t_n(s;h): n\in\mathcal{N}\}$ denote the set of RMIs associated with all $N$ arms in time slot $h$,  
and we prioritize the arms according to a decreasing order of their RMIs, and then activate the $B$ arms with the highest indices. The RMI policy $\pi^{t,\star}:=\{\pi_{n}^{t,\star}, \forall n\}$ will be executed the entire episode $t$.  Note that the proposed RMI index policy is majorly distinct from the stochastic RMAB setting in terms of the inclusion of reward. Since the rewards are adversarially determined, in our proposed RMI index, we do not contain the reward in our index as \citep{xiong2022AAAI, xiong2022Neurips} did for stochastic settings. Still, we are able to show that the proposed RMI index is asymptotically optimal in the following theorem.
 

\begin{theorem}\label{thm:asympt_opt}
The proposed RMI policy is asymptotic optimal when the number of each type of arm and the budget is enlarged by $\rho$ times with $\rho\rightarrow\infty$.
\end{theorem}


\begin{remark}
Conventional research  primarily concentrates on devising stationary policies derived from the occupancy measure. This approach is tailored to the context of a single MDP, where the stationary policy framework proves effective.
In contrast, our work is distinctly oriented toward regret minimization in adversarial  RMAB scenarios characterized by multiple MDPs and a stringent "hard" activation constraint. In this complex setting, the traditional stationary policy approach falls short of addressing the challenges at hand. Consequently, our research shifts its focus towards the development of time-dependent index policies. This explains the difference of our occupancy measure definitions in \eqref{eq:OM}.
\end{remark}





==> Related_work.tex <==

\section{related work}
In this section, we present the related works from three different categories, i.e.,  adversarial MDPs, online learning in CMDPs, and RMABs, and summarize the model difference with previous work in Table  \ref{table:1}.



\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Related Work & Model & Feedback & Constraint & Algorithm & Regret \\
\hline \citep{rosenberg2019online}& MDP &  \emph{Full} & \ding{55} & OMD & $\mathcal{O}(\sqrt{T})$\\ \hline
\citep{rosenberg2019b} & MDP & \emph{Bandi}t & \ding{55}& OMD & $\mathcal{O}(T^{3/4})$\\
\hline
\citep{jin2020learning} & MDP & \emph{Bandit} & \ding{55} & OMD & $\mathcal{O}(\sqrt{T})$ \\ \hline
\cite{qiu2020upper} & CMDP & \emph{Full} & \emph{Stochastic} & Primal-dual& $\mathcal{O}(\sqrt{T})$\\
\hline
\citep{germano2023best} & CMDP & \emph{Full} & \emph{Stochastic} & Primal-dual& $\mathcal{O}(\sqrt{T})$\\
\hline
\citep{luo2021policy} & MDP & \emph{Bandit} & \ding{55} & Policy Opt. & $\mathcal{O}(\sqrt{T})$\\
\hline
\textbf{This Work} & \textbf{RMAB} & \emph{Bandit} & \textbf{Hard} & \textbf{Index-based}&${\mathcal{O}(\sqrt{T})}$\\
\hline
\end{tabular}
\caption{Comparison of existing work with adversarial loss (reward) and unknown transitions.}
\label{table:1}
\end{table}
\textbf{Adversarial MDP.}
Markov Decision processes (MDPs) \citep{puterman1994markov} are widely used for modeling sequential decision-making in stochastic environments. However, real-world applications can involve dynamic losses that change over time during the learning process.
The adversarial MDP model \citep{even2009online} addresses these challenges by allowing for arbitrary changes in the loss (reward) function while assuming a fixed stochastic transition function. The learner's goal is to minimize average loss, measured by regret relative to the best stationary policy in hindsight.  

\citep{neu2012adversarial} first formulated this problem as a shortest-path problem under the framework of full-information feedback of adversarial loss functions with unknown transitions. It combines Follow- the- Perturbed- Optimistic Policy desined for bandits problem and a confidence set of transition functions,  resulting in a regret bound of $\tilde{\mathcal{O}}(L|\cS||\cA|\sqrt{T})$, where L represents the steps of each episode, $|\cS|$ is the state space cardinality, $|\cA|$ is the action space cardinality, and $T$ is the number of episodes. This problem is reviewed recently by \citep{rosenberg2019online}, which proposed a UCRL2-based online optimization algorithm under full information feedback and unknown transitions and achieved $\tilde{\mathcal{O}}(L|\cS|\sqrt{|\cA|T}).$ Later on, \citep{rosenberg2019b} extended the full-information feedback setting to a more challenged setting where the adversarial losses are of bandit feedback and thus need to be estimated. It hence achieved a regret of order $\tilde{\mathcal{O}}(L^{3/2}|\cS||\cA|^{1/4}T^{3/4})$.  Under the same setting, \citep{jin2020learning} proposed a novel reward estimator and a modified radius of upper confidence ball, which pushed the regret back to the order $\tilde{\mathcal{O}}(L|\cS|\sqrt{|\cA|T}).$ \citep{luo2021policy}also follows this bandit feedback setting and proposes a different policy optimization technique which still guarantees the  $\tilde{\mathcal{O}}(\sqrt{T})$ regret order.
  
Recently, there are some related adversarial MDP work but with some modifications. For example, 
\citep{jin2021best} considered the best-of-both-worlds setting, which designed an algorithm working for both stochastic and adversarial losses. 
\citep{jin2022near} considered the setting with delayed bandit feedback, and
\citep{jin2023no} considered the setting where both loss functions and transitions are both determined by the adversary. Though the considered settings in \citep{jin2021best, jin2022near, jin2023no} are more challenging than the conventional adversarial setting, theoretical results have shown that the $\mathcal{O}(\sqrt{T})$ regret order is still achievable. 
 



\textbf{Online Learning in CMDP.}
Past investigations in this domain have predominantly centered around settings with stochastic loss (reward) functions and stochastic constraints with unknown transitions. For example, the work of \citep{zheng2020constrained} delved into episodic CMDPs featuring stochastic losses and constraints. In this context, the transition probabilities were assumed to be known, and feedback followed a bandit paradigm. Their algorithm yielded a regret upper bound on the order of $\tilde{\mathcal{O}}
(T^{3/4})$ which is suboptimal in terms of $T$, alongside a guarantee of maintaining cumulative constraint violation below a predefined threshold. In parallel, \citep{efroni2020exploration} conducted a concurrent study on episodic MDPs featuring unknown transitions and stochastic bandit feedback for both losses and constraints. Their approach resulted in achieving an $\tilde{\mathcal{O}}(\sqrt{T})$ regret and constraint violation. In a separate investigation, \citep{ding2021provably} explored constrained episodic MDPs characterized by a linear structure and adversarial losses. They employed a primal-dual-type policy optimization algorithm, which led to the attainment of an $\tilde{\mathcal{O}}(\sqrt{T})$ regret and constraint violation.\cite{qiu2020upper} proposed a primal-dual approach grounded in optimism under uncertainty for addressing episodic CMDPs with adversarial losses and stochastic constraints. It achieves sublinear regret and constraint violation while utilizing full-information feedback.
Most recently, \cite{germano2023best} considered the first work that both reward functions and constraints are adversarial and proposed a best-of-both-world algorithm, which only achieves $\tilde{\mathcal{O}}(T^{3/4})$ regret and constraint violation. 

\textbf{Restless Multi-Armed Bandits.}
The RMAB problem is a general model for a variety
of sequential decision-making problems which are notoriously intractable\citep{papadimitriou1994complexity} and Whittle proposed a heuristic called the Whittle index for the
infinite-horizon RMAB \cite{whittle1988restless}. Inspired by Whittle, many following studies focus on finding index policies for RMAB problems \citep{verloop2016asymptotically}. However, the unknown transitions and rewards functions give rise to a bunch of online learning-based techniques \cite{liu2012learning, ortner2012regret, wang2020restless, xiong2022AAAI, xiong2022Neurips}. 
In particular, \citep{liu2012learning} may not perform close to the offline optimal as the baseline policy is often heuristic without a performance guarantee, making the
regret $\tilde{\mathcal{O}}(\log T)$ less meaningful. Colored-UCRL2 in\citep{ortner2012regret} guarantees the $\tilde{\mathcal{O}}(\sqrt{T})$ while suffers from an exponential computation complexity. \cite{wang2020restless} proposed a generative model-based algorithm to learn the Whittle index, which is simple in complexity, but can only achieve a regret with order $\tilde{\mathcal{O}}(T^{2/3})$. \cite{xiong2022AAAI,xiong2022Neurips} proposed a novel index policy and learn the proposed index policy for both finite-horizon and infinite-horizon, which is both computationally efficient and can guarantee $\tilde{\mathcal{O}}(\sqrt{T})$ regret. 
Need to mention that all the current related work on RMAB focuses on the stochastic setting where the reward functions are stochastically sampled from a fixed distribution. To our best knowledge, this is the first work that study RMAB in adversarial settings.





==> System_model.tex <==
\section{System Model and Problem Formulation}\label{sec:model}
Consider an episodic adversarial restless multi-armed bandit (RMAB) problem with $N$ arms. Each arm $n$ is associated with a specific unichain markov decision process (MDP)  denoted by a tuple $(\cS, \cA, P_n, H, \{r_n^t, \forall t\in[T]\})$, where 
\begin{itemize}
    \item $T$ is a number of episodes, with $t\in[T]$ being a specific episode\footnote{We denote [T] as the set of consecutive integers from $1$ to $T$.}; and $H$ is the length of each episode.
    \item $\cS$ is the finite state space, and $\cA:=\{0,1\}$ denotes the set of binary actions. Using the standard terminology from the RMAB literature, we call an arm \textit{passive} when action $a=0$ is applied to it, and \textit{active} otherwise.
    \item $P_n:\cS\times\cA\times\cS\mapsto[0,1]$ is the transition kernel with $P_n(s^\prime|s,a)$ being the probability of transition to state $s^\prime$ from state $s$ by taking action $a$.
    \item $r_n^t: \cS\times\cA\mapsto [0,1]$ is the reward function\footnote{Though most existing work on adversarial online learning setting use the term ``losses'' instead of ``rewards", we still use "reward" in this paper as it is commonly used in RMAB literature. These two terms are equivalent by simply taking the negation of any one of them.} for episode $t$, which is determined by an adversary. W.o.l.g., we assume that $r_n(s,0)=0, \forall s\in\cS, n\in[N]$.   
\end{itemize}
 For a standard RMAB problem,  the total number of active arms at each time slot $h$ of episode $t$ is constrained by $B$, i.e., $\sum_{n} A_n^{t,h}\leq B$, which we call the \textit{activation budget.}
For any episode $t$, a policy $\pi^t:\cS^N\rightarrow\cA^N$ indicates the action $a\in\cA$ the decision maker (DM) to choose at any give state $s \in\cS$ for all $N$ arms. Let $\{(S_n^{t,h}, A_n^{t,h})\in\cS\times \cA, \forall n\in[N]\}$ denotes the random tuples generated according to the transition kernels $\{P_n, \forall n\in[N]\}$ and the policy $\pi^t$. The corresponding expected reward in episode $t$ is 
\begin{align}
   R_t:= \mathbb{E}\left[\sum_{h=1}^{H}\sum_{n=1}^N r_n^t(S_n^{t,h},A_n^{t,h})\Big|\{P_n, \forall n\in[N]\}, \pi^t\right].
\end{align}


\begin{remark}
Notice that existing work for adversarial MDP \citep{rosenberg2019online,rosenberg2019b, jin2020learning} and CMDP setting \citep{qiu2020upper}
assumes that the state space is loop-free such that it can be divided into distinct $K$ layers, i.e., $\cS:=\cS_1\cup\cS_2\cup\ldots\cup\cS_K$ with a singleton initial layer $\cS_1=\{s_1\}$ and terminal layer $\cS_K=\{s_K\}$, and $\cS_k \cap \cS_j=\emptyset, j\neq k.$ Transitions are only occurred between consecutive layers, which is $P(s^\prime|s,a)>0$ if $s^\prime \in \cS_{k+1}, s\in\cS_k, \forall k\in\{1,\ldots, K\}$.  This 
assumption enforces that each path from the initial state to the terminal state takes a fixed length $K$.  {However, this is an excessively restrictive assumption as any non-loop-free MDP with episode length being $K$ needs to extend the state space $K$ times to be transformed into one with a fixed path length $K$, which enlarges the regret at least $K$ times.  In most real-world applications, the considered MDP is not loop-free. Therefore, we do not assume this loop-free MDP in this paper.}


\end{remark}

\begin{remark}
   The major setting difference between adversarial MDPs and stochastic MDPs is that stochastic MDPs involve rewards that follow a constant
stochastic distribution across episodes, while adversarial MDPs feature rewards determined by an adversarial
agent, varying from episode to episode due to the adversarial nature of the environment. This gives rise to a
significantly different objective as the DM must adapt to dynamic and potentially hostile reward structures
while striving to find an optimal policy across all episodes.

\end{remark}

\subsection{Offline Adversarial RMAB Optimization}
The goal of DM is to maximize the total expected reward over $T$ episodes under the hard budget constraint that the number of activated arms should not exceed budget $B$, i.e.,
\begin{align}
 &\qquad\max_\pi \sum_{t=1}^T R_t, 
 ~~\text{s.t.} \sum_{n=1}^N A_n^{t,h}\leq B, \forall h\in [H] ,t\in [T].
    \label{eq:orginal_P}
\end{align}
It means that DM needs to find {\color{red} a single optimal policy $\pi:=\{\pi_h(a|s),\forall s\in\cS, a\in\cA, h\in[H]\}$ for } \eqref{eq:orginal_P} with $T$ episodes, and we define it as $\pi^{opt}$ for simplicity. 
Notice that even when the underlying MDP (i.e., transition kernel) of each arm is known and the adversarial rewards are known in hindsight, the problem~(\ref{eq:orginal_P}) can only be solved using relative value iteration \citep{puterman1994markov,bertsekas1995dynamic} in theory. Unfortunately, this approach suffers from the curse of dimensionality \citep{bertsekas1995dynamic}, and lacks insights for the solution structure. This property is fundamentally different from adversarial MDP and CMDP problems where only one MDP exists \citep{rosenberg2019online,rosenberg2019b, jin2020learning} .
Moreover, assuming the full information of MDPs and the adversarial rewards in advance is not practical in most scenarios.  These challenges lead to the online framework for solving \eqref{eq:orginal_P}.

\subsection{Online Setting and Learning Regret}


\begin{algorithm}[h]
	\caption{{Online Interaction between Decision-Maker and Adversarial RMAB Environment}}
	\label{alg:importance-policy}
	\begin{algorithmic}[1]
		\REQUIRE {\color{red} State space $\cS$, action space $\cA=\{0,1\}$, and unknown transitions  $\{\cP_n, n\in[N]\}$;}
  \FOR{$t=1$ to $T$}
\STATE All arms start in state $S_n^{t,1}, \forall n\in[N]$ according to {\color{red} distribution $\bs_1(s), \forall s\in\cS$;}
\STATE Adversary decides the reward function $\{r_n^t, \forall n\in[N]\}$ for this episode;
\STATE DM decides a policy $\pi^t$ for this episode; 
  \FOR{$h=1$ to $H$}
  \STATE DM chooses actions $\{A_{n}^{t,h}, \forall n\in [N]\}$ such that $\sum_{n=1}^N A_{n}^{t,h}=B$;
  \STATE DM observes reward function $\{r_n^t(S_n^{t,h}, A_n^{t,h}), \forall n\in[N]\}$;
  \STATE Arm $n, \forall n \in[N]$ moves to the next state $S_n^{t,h+1}\sim P_n(\cdot|S_n^{t,h},A_n^{t,h})$ ;
  \STATE DM observes states $\{S_n^{t,h+1}, \forall n\in[N]\}$;
  \ENDFOR
  
	 \ENDFOR 
		
		
	\end{algorithmic}
\end{algorithm}

We focus on the online adversarial setting where the underlying MDPs are unknown and the adversarial reward is of bandit-feedback\footnote{We use the same term "bandit-feedback" with existing work to denote that only the reward of visited state-action pairs is revealed at the end of each episode. Notice that the "bandit" term in "bandit-feedback" is different from the "bandit" in the RMAB problem.  }.
At the beginning of each episode $t$, the DM determines a policy $\pi_t$ and executes this policy for the entire episode. The DM interacts with the environment as follows. 
For each step $h$ at episode $t$, the DM chooses actions $\{A_{n}^{t,h}, \forall n\in \cN\}$ according to $\pi_t$ such that $\sum_{n=1}^N A_{n}^{t,h}=B$; and arm $n, \forall n \in\cN$ moves to the next state $S_n^{t,h+1}\sim P_n(\cdot|S_n^{t,h},A_n^{t,h})$. The DM records the trajectory of the current episode $t$ and the rewards of the visited state-action pair are observed at the end of episode $t$. The details are summarized in Algorithm \ref{alg:importance-policy}.

  Specifically, for the total $T$ episodes, we denote the expected cumulative reward under the learned policy sequence $\{\pi^t, \forall t\in[T]\}$ {\color{red}given the initial states $\bs_1$ as} 
\begin{align}
    R(\bs_1, T, \{\pi^t, \forall t\}):={\color{red}\sum_{t=1}^{T} R_t= }\mathbb{E}\left[\sum_{t=1}^T\sum_{h=1}^{H}\sum_{n=1}^N r_n^t(s_n^{t,h},a_n^{t,h})\Big|\{P_n, \forall n\}, \{\pi^t, \forall t\}\right],
\end{align}
which is a random variable. Let the optimal expected reward be $$R(\bs_1, T, \pi^{opt}):=\mathbb{E}\left[\sum_{t=1}^T\sum_{h=1}^{H}\sum_{n=1}^N r_n^t(s_n^{t,h},a_n^{t,h})\Big|\{P_n, \forall n\}, \pi^{opt}\right].$$ 


The goal of the DM for the online setting is to minimize the learning regret, which
is defined as the expected gap between the offline optimum, i.e.,
the best policy under full knowledge of all transition probabilities and reward information, and the cumulative reward obtained
by the learned policy.
Then the regret of $\{\pi^t, \forall t\in[T]\}$ is defined as \footnote{Though the regret definition looks similar to that in the stochastic setting, the fundamental difference is that $\pi^{opt}$ in \eqref{eq:regret} is only optimal for the total $T$ episodes, not optimal for every single episode as the optimal policy under stochastic setting is. Hence, regret does not necessarily occur in every episode as opposed to the stochastic settings. This leads to a significant difference in terms of regret characterization under an adversarial setting compared with a stochastic one.}
\begin{align}\label{eq:regret}
    \Delta(T):=R(\bs_1, T, \pi^{opt})-R(\bs_1, T, \{\pi^t, \forall t\in[T]\}).
\end{align}


In the realm of conventional adversarial MDPs \citep{rosenberg2019online, jin2020learning} and CMDPs\citep{qiu2020upper}, a common approach involves the initial establishment of an occupancy measure (i.e., a probability measure),  and then transforming the problem of minimizing regret, as depicted in \eqref{eq:regret}, into an equivalent one that is intricately connected with the occupancy measure.
However, it needs to underscore a fundamental difference from this standard paradigm within the context of the considered regret minimization in an adversarial RMAB setting, where the mathematical expectation over policy outcomes does not exhibit equivalence with the occupancy measure. The underlying reason behind this is that for the RMAB setting, the policy is not stationary as those in MDP and CMDP settings. We relegate the details in Section \ref{sec:learning}.

% {\color{red}  When the underlying MDPs are not known, off-the-shelf RL algorithms are either computationally expensive or without an $\tilde{\cO}(\sqrt{T})$ regret guarantee.  
% We overcome this
% difficulty by developing an index-based policy that is computationally appealing and provably optimal.
% In the remainder of the paper, we first build a low-complexity index based policy for~(\ref{eq:orginal_P}) with optimality guarantee when the MDPs are known in Section~\ref{sec:indexpolicy}, and then design index-aware RL algorithms for~(\ref{eq:orginal_P}) that not only are computationally efficient but also achieve an $\tilde{\cO}(\sqrt{T})$ regret when the MDPs are unknown in Section~\ref{sec:learning}.} 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

